Uniform spectral asymptotics for semiclassical wells on phase space loops

We consider semiclassical self-adjoint operators whose symbol, defined on a two-dimensional symplectic manifold, reaches a non-degenerate minimum $b_0$ on a closed curve. We derive a classical and quantum normal form which allows us, in addition to the complete integrability of the system, to obtain eigenvalue asymptotics in a window $(-\infty,b_0+\epsilon]$ for $\epsilon > 0$ independent on the semiclassical parameter. These asymptotics are obtained in two complementary settings: either a symmetry of the system under translation along the curve, or a Morse hypothesis reminiscent of Helffer-Sj\"ostrand's "miniwell" situation.

==> macro.tex <==
\RequirePackage{amsmath,amsthm,amsfonts,amssymb}

\newcommand{\RM}{\mathbb{R}}
\newcommand{\ZM}{\mathbb{Z}}
\newcommand{\QM}{\mathbb{Q}}
\newcommand{\NM}{\mathbb{N}}
\newcommand{\CM}{\mathbb{C}}
\newcommand{\SM}{\mathbb{S}}
\newcommand{\Cinf}{C^\infty}


\newcommand{\theor}{Theorem}
\newcommand{\defin}{Definition}
\newcommand{\lemma}{Lemma}
\newcommand{\remar}{Remark}
\newcommand{\exemp}{Example}
\newcommand{\corol}{Corollary}
\newcommand{\propo}{Proposition}
\newcommand{\demon}{Proof}
\newcommand{\probl}{Problem}
\newcommand{\exam}{Example}

\newtheorem{theo}{\theor}[section]
\newtheorem{theo*}{\theor}
% ancienne version (jusqu'au 22 mai 2003:)
% \newtheorem{defi}{\defin}[section]
% maintenant on numerote tout sequentiellement
\newtheorem{prop}[theo]{\propo}
\newtheorem{lemm}[theo]{\lemma}
\newtheorem{coro}[theo]{\corol}
\newtheorem{conj}[theo]{Conjecture}
%\newtheorem{prob}{Problem}[section]
\newtheorem{prob}{\probl}[section]
\newtheorem{assu}{Assumption}

\theoremstyle{definition}
\newtheorem{defi}[theo]{\defin}
\newtheorem{defi*}[theo*]{\defin}
\newtheorem{rema}[theo]{\remar}
\newtheorem{ex}[theo]{\exam}

\newcommand{\phy}{\varphi}
\newcommand{\epsi}{\varepsilon}
\newcommand{\bep}{\mbold{\epsilon}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\om}{\omega}
\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}
\newcommand{\cqfd}{\hfill $\square$\par\vspace{1ex}}
\newcommand{\h}{\hbar}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\bigO}{\mathcal{O}}

\newcommand{\ad}[1]{{\operatorname{ad}}_{#1}}
\newcommand{\Ad}[1]{{\operatorname{Ad}}_{#1}}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}

\newcommand{\restr}{\upharpoonright}


\newcommand{\demons}[1][$\!\!$]{\noindent\textbf{\demon\ }\textsl{#1}\textbf{.}~}
\newenvironment{demo}[1][$\!\!$]
{\demons[#1]\ }
{\cqfd}
